Energy exchanges between atoms with a quartz crystal $\mu$-balance

We propose an experimental method to fully characterize the energy exchange of particles during the physical vapor deposition process of thin surface layers. Our approach is based on the careful observation of perturbations of the oscillation frequency of a Quartz Crystal $\mu$-balance induced by the particles interaction. With this technique, it is possible to measure the momentum exchange of the atoms during the evaporation process and determine the ideal evaporation rate for an uniform energy distribution. We are able to follow the desorption dynamics of particles immediately after the first layers have been formed. These results are in close relation to the surface binding energy of the evaporated material, they offer a better control to obtain the desired properties of the thin surface layer. We applied our technique to investigate the physical vapor evaporation process for diverse elements, usually implemented in the development of film surface layers, such as Cu, W, Au, Gd and In, and confirm that our results are in agreement with measurements done previously with other techniques such as low-temperature photoluminescence.

==> refs.tex <==
@article{clark2014polycrystalline,
  title={Polycrystalline indium films in the percolation threshold regime: time correlation between electric conduction and optical properties with film morphology},
  author={Clark, Neville and Vargas, William E and Azofeifa, Daniel E and S{\'a}enz-Arce, Giovanni and Sol{\'\i}s, Hugo and Ram{\'\i}rez-Hidalgo, Gustavo},
  journal={Materials Research Express},
  volume={1},
  number={1},
  pages={016302},
  year={2014},
  publisher={IOP Publishing}
}

@article{Lewandowski-2003,
year={2003},
issn={0022-2291},
journal={Journal of Low Temperature Physics},
volume={132},
number={5-6},
doi={10.1023/A:1024800600621},
title={Simplified System for Creating a Bose–Einstein Condensate},
url={http://dx.doi.org/10.1023/A%3A1024800600621},
publisher={Kluwer Academic Publishers-Plenum Publishers},
keywords={Bose–Einstein condensation; experimental apparatus; magnetic trap; degenerate gas},
author={Lewandowski, H.J. and Harber, D.M. and Whitaker, D.L. and Cornell, E.A.},
pages={309-367},
language={English}
}

@ARTICLE{Zhao-2014,
   author = {{Zhao}, L. and {Jiang}, J. and {Liu}, Y.},
    title = "{Optimizing a spin-flip Zeeman slower}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1401.7181},
 primaryClass = "cond-mat.quant-gas",
 keywords = {Condensed Matter - Quantum Gases, Physics - Atomic Physics},
     year = 2014,
    month = jan,
   adsurl = {http://adsabs.harvard.edu/abs/2014arXiv1401.7181Z},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{Courtillot-2003, 
author = {I. Courtillot and A. Quessada and R. P. Kovacich and J-J. Zondy and A. Landragin and A. Clairon and P. Lemonde}, 
journal = {Opt. Lett.}, 
keywords = {Laser trapping; Laser cooling; Harmonic generation and mixing},
number = {6}, 
pages = {468--470}, 
publisher = {OSA},
title = {Efficient cooling and trapping of strontium atoms}, 
volume = {28}, 
month = {Mar},
year = {2003},
url = {http://ol.osa.org/abstract.cfm?URI=ol-28-6-468},
doi = {10.1364/OL.28.000468},

}

@article{Phillips-1982,
  title = {Laser Deceleration of an Atomic Beam},
  author = {Phillips, William D. and Metcalf, Harold},
  journal = {Phys. Rev. Lett.},
  volume = {48},
  issue = {9},
  pages = {596--599},
  numpages = {0},
  year = {1982},
  month = {Mar},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.48.596},
  url = {http://link.aps.org/doi/10.1103/PhysRevLett.48.596}
}

@article{Bober-2010,
   author = {{Bober}, M. and {Zachorowski}, J. and {Gawlik}, W.},
    title = "{Designing Zeeman slower for strontium atoms - towards optical atomic clock}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1006.1554},
 primaryClass = "physics.atom-ph",
 keywords = {Physics - Atomic Physics},
     year = 2010,
    month = jun,
   adsurl = {http://adsabs.harvard.edu/abs/2010arXiv1006.1554B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{Kondo-1997,
  author={Yoshiteru Kondo and Mitsuyo Saito and Masafumi Yamashita and Toshiharu Tako  and Atsuo Morinaga},
  title={Influence of the Magnetic Field Gradient on the Extraction of Slow Sodium Atoms outside the Solenoid in the Zeeman Slower},
  journal={Japanese Journal of Applied Physics},
  volume={36},
  number={2R},
  pages={905},
  url={http://stacks.iop.org/1347-4065/36/i=2R/a=905},
  year={1997},
  abstract={In order to produce an intense steady flux of slow sodium atoms outside the solenoid in a Zeeman slower, the relation between the extraction velocity of the atoms and the magnetic field gradient at the exit of the Zeeman solenoid was examined. When the magnetic field gradient was 0.5 T/m, slow atoms with a velocity of 160 m/s were extracted outside the solenoid with a slowing laser detuning of 250 MHz. On the other hand, when the magnetic field gradient was higher, i.e., 1.4 T/m, slow atoms with a velocity of 30 m/s were extracted with a slowing laser detuning of 550 MHz. The magnetic-field adiabatic following condition is discussed by comparing the experimental results with those of a Monte Carlo simulation.}
}

@article{Prodan-1982,
  title = {Laser Production of a Very Slow Monoenergetic Atomic Beam},
  author = {Prodan, John V. and Phillips, William D. and Metcalf, Harold},
  journal = {Phys. Rev. Lett.},
  volume = {49},
  issue = {16},
  pages = {1149--1153},
  numpages = {0},
  year = {1982},
  month = {Oct},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.49.1149},
  url = {http://link.aps.org/doi/10.1103/PhysRevLett.49.1149}
}

@mastersthesis{Harris-2003,
  author       = {Margareth Lynn Harris}, 
  title        = {Design and construction of an improved Zeeman Slower},
  school       = {Duke University},
  year         = 2003

}

@mastersthesis{Herrera-2008,
  author       = { Herrera-Sancho,\'Oscar Andrey}, 
  title        = {Growth and characterization of two-dimensional nanostructures},
  school       = {University of Costa Rica},
  year         = 2008

}

@ARTICLE{Herrera-2011,
   author = {Herrera-Sancho, O.A. and Castro-Gonz{\'a}lez, D. and Araya-Pochet, J.A. and 
	Vargas-Castro, W.E.},
    title = {Ultra thin films of gadolinium deposited by evaporation in ultra high vacuum conditions: Composition, growth and morphology},
  journal = {Applied Surface Science},
     year = 2011,
    month = feb,
   volume = 257,
    pages = {3510-3518},
      doi = {10.1016/j.apsusc.2010.11.065},
   adsurl = {http://adsabs.harvard.edu/abs/2011ApSS..257.3510H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@book{vanhove-2012,
  title={Low-energy electron diffraction: experiment, theory and
surface structure determination},
  author={VanHove, Michel A and Weinberg, William Henry and Chan, Chi-Ming},
  volume={6},
  year={2012},
  publisher={Springer Science \& Business Media}
}

@article{Davisson-1928,
  title={Reflection of electrons by a crystal of nickel},
  author={Davisson, CJ and Germer, LH},
  journal={Proceedings of the National Academy of Sciences of the United States of America},
  volume={14},
  number={4},
  pages={317},
  year={1928},
  publisher={National Academy of Sciences}
}

@article{Bragg-1913,
  title={The reflection of X-rays by crystals},
  author={Bragg, WH and Bragg, WL},
  journal={Proceedings of the Royal Society of London. Series A, Containing Papers of a Mathematical and Physical Character},
  pages={428--438},
  year={1913},
  publisher={JSTOR}
}

@book{Membranes-2011,
  title={Membranes Surfaces Boundaries},
Author={Grote, Mathias and Stadler, Max},
  volume={420},
  year={2011},
  publisher={Max-Planck-Inst. f{\"u}r Wissenschaftsgeschichte}
}

@article{kasemo-2002,
  title={Biological surface science},
  author={Kasemo, Bengt},
  journal={Surface science},
  volume={500},
  number={1},
  pages={656--677},
  year={2002},
  publisher={Elsevier}
}

@article{Campos-2011,
  title={Visible light reflection spectra from cuticle layered materials},
  author={Campos-Fern{\'a}ndez, Cristian and Azofeifa, Daniel E and Hern{\'a}ndez-Jim{\'e}nez, Marcela and Ruiz-Ruiz, Adams and Vargas, William E},
  journal={Optical Materials Express},
  volume={1},
  number={1},
  pages={85--100},
  year={2011},
  publisher={Optical Society of America}
}

@article{Fink-1990,
  title={Experimental probe for thin-film magnetism in p (1$\times$ 1) Pd and V on Ag (100)},
  author={Fink, RL and Ballentine, CA and Erskine, JL and Araya-Pochet, Jose A},
  journal={Physical Review B},
  volume={41},
  number={14},
  pages={10175},
  year={1990},
  publisher={APS}
}

@article{Cohen-1984,
  title={Electronic properties of surfaces},
  author={Cohen, Marvin L and Louic, SG},
  journal={Annual Review of Physical Chemistry},
  volume={35},
  number={1},
  pages={537--562},
  year={1984},
  publisher={Annual Reviews 4139 El Camino Way, PO Box 10139, Palo Alto, CA 94303-0139, USA}
}

@article{jasik2009influence,
  title={The influence of the growth rate and V/III ratio on the crystal quality of InGaAs/GaAs QW structures grown by MBE and MOCVD methods},
  author={Jasik, A and Wnuk, A and Gaca, J and W{\'o}jcik, M and W{\'o}jcik-Jedli{\'n}ska, A and Muszalski, J and Strupi{\'n}ski, W},
  journal={Journal of Crystal Growth},
  volume={311},
  number={19},
  pages={4423--4432},
  year={2009},
  publisher={Elsevier}
}
@article{jackson-1974,
  title={Approximate calculation of surface Debye temperatures},
  author={Jackson, DP},
  journal={Surface Science},
  volume={43},
  number={2},
  pages={431--440},
  year={1974},
  publisher={Elsevier}
}

@article{ferry-1996,
  title={Observation of the second ordered phase of water on the MgO (100) surface: Low energy electron diffraction and helium atom scattering studies},
  author={Ferry, D and Glebov, A and Senz, V and Suzanne, J and Toennies, JP and Weiss, H},
  journal={The Journal of chemical physics},
  volume={105},
  number={4},
  pages={1697--1701},
  year={1996},
  publisher={AIP Publishing}
}

@article{mahan2000physical,
  title={Physical vapor deposition of thin films},
  author={Mahan, John E},
  journal={Physical Vapor Deposition of Thin Films, by John E. Mahan, pp. 336. ISBN 0-471-33001-9. Wiley-VCH, January 2000.},
  pages={336},
  year={2000}
}



@article{Heinz-1995,
  title={LEED and DLEED as modern tools for quantitative surface structure determination},
  author={Heinz, Klaus},
  journal={Reports on Progress in Physics},
  volume={58},
  number={6},
  pages={637},
  year={1995},
  publisher={IOP Publishing}
}

@article{blum-2001,
  title={Fast LEED intensity calculations for surface crystallography using Tensor LEED},
  author={Blum, V and Heinz, K},
  journal={Computer physics communications},
  volume={134},
  number={3},
  pages={392--425},
  year={2001},
  publisher={Elsevier}
}

@article{pendry-1993,
  title={LEED and the crystallography of surfaces},
  author={Pendry, JB},
  journal={Surface science reports},
  volume={19},
  number={3},
  pages={87--97},
  year={1993},
  publisher={Elsevier}
}

@article{Tannoudji-1998,
  title={Nobel Lecture: Manipulating atoms with photons},
  author={Cohen-Tannoudji, Claude N},
  journal={Reviews of Modern Physics},
  volume={70},
  number={3},
  pages={707},
  year={1998},
  publisher={APS}
}

@article{Ketterle-2002,
  title={Nobel lecture: When atoms behave as waves: Bose-Einstein condensation and the atom laser},
  author={Ketterle, Wolfgang},
  journal={Reviews of Modern Physics},
  volume={74},
  number={4},
  pages={1131},
  year={2002},
  publisher={APS}
}

@book{Boyd-2007,
  title={High precision spectroscopy of strontium in an optical lattice: Towards a new standard for frequency and time},
  author={Boyd, Martin M},
  year={2007},
  publisher={ProQuest}
}

@article{Xu-2003,
  title={Cooling and trapping of atomic strontium},
  author={Xu, Xinye and Loftus, Thomas H and Hall, John L and Gallagher, Alan and Ye, Jun},
  journal={JOSA B},
  volume={20},
  number={5},
  pages={968--976},
  year={2003},
  publisher={Optical Society of America}
}

@techreport{stellmer-2013,
  title={Degenerate quantum gases of strontium},
  author={Stellmer, Simon and Schreck, Florian and Killian, Thomas C},
  year={2013},
  institution={World Scientific}
}

@article{Escobar-2009,
  title={Bose-Einstein Condensation of Sr 84},
  author={de Escobar, YN Martinez and Mickelson, PG and Yan, M and DeSalvo, BJ and Nagel, SB and Killian, TC},
  journal={Physical review letters},
  volume={103},
  number={20},
  pages={200402},
  year={2009},
  publisher={APS}
}

@article{stellmer-2009,
  title={Bose-Einstein condensation of strontium},
  author={Stellmer, Simon and Tey, Meng Khoon and Huang, Bo and Grimm, Rudolf and Schreck, Florian},
  journal={Physical review letters},
  volume={103},
  number={20},
  pages={200401},
  year={2009},
  publisher={APS}
}

@article{daley-2008,
  title={Quantum computing with alkaline-earth-metal atoms},
  author={Daley, Andrew J and Boyd, Martin M and Ye, Jun and Zoller, Peter},
  journal={Physical review letters},
  volume={101},
  number={17},
  pages={170504},
  year={2008},
  publisher={APS}
}

@article{gorshkov-2010,
  title={Two-orbital SU (N) magnetism with ultracold alkaline-earth atoms},
  author={Gorshkov, AV and Hermele, M and Gurarie, V and Xu, C and Julienne, PS and Ye, J and Zoller, P and Demler, E and Lukin, MD and Rey, AM},
  journal={Nature Physics},
  volume={6},
  number={4},
  pages={289--295},
  year={2010},
  publisher={Nature Publishing Group}
}

@article{Morsch-2006,
  title={Dynamics of Bose-Einstein condensates in optical lattices},
  author={Morsch, Oliver and Oberthaler, Markus},
  journal={Reviews of modern physics},
  volume={78},
  number={1},
  pages={179},
  year={2006},
  publisher={APS}
}


@article{phillips-1998,
  title={Nobel Lecture: Laser cooling and trapping of neutral atoms},
  author={Phillips, William D},
  journal={Reviews of Modern Physics},
  volume={70},
  number={3},
  pages={721},
  year={1998},
  publisher={APS}
}

@article{Barry-2012,
  title={Laser radiation pressure slowing of a molecular beam},
  author={Barry, JF and Shuman, ES and Norrgard, EB and DeMille, D},
  journal={Physical review letters},
  volume={108},
  number={10},
  pages={103002},
  year={2012},
  publisher={APS}
}

@article{Cornell-2002,
  title={Nobel Lecture: Bose-Einstein condensation in a dilute gas, the first 70 years and some recent experiments},
  author={Cornell, Eric A and Wieman, Carl E},
  journal={Reviews of Modern Physics},
  volume={74},
  number={3},
  pages={875},
  year={2002},
  publisher={APS}
}
@article{Petsas-1994,
  title={Crystallography of optical lattices},
  author={Petsas, KI and Coates, AB and Grynberg, G},
  journal={Physical review A},
  volume={50},
  number={6},
  pages={5173},
  year={1994},
  publisher={APS}
}

@article{Greiner-2001,
  title={Exploring phase coherence in a 2D lattice of Bose-Einstein condensates},
  author={Greiner, Markus and Bloch, Immanuel and Mandel, Olaf and H{\"a}nsch, Theodor W and Esslinger, Tilman},
  journal={Physical Review Letters},
  volume={87},
  number={16},
  pages={160405},
  year={2001},
  publisher={APS}
}

@article{Bloch-2008,
  title={Many-body physics with ultracold gases},
  author={Bloch, Immanuel and Dalibard, Jean and Zwerger, Wilhelm},
  journal={Reviews of Modern Physics},
  volume={80},
  number={3},
  pages={885},
  year={2008},
  publisher={APS}
}

@article{Moses-2015,
  title={Creation of a low-entropy quantum gas of polar molecules in an optical lattice},
  author={Moses, Steven A and Covey, Jacob P and Miecnikowski, Matthew T and Yan, Bo and Gadway, Bryce and Ye, Jun and Jin, Deborah S},
  journal={Science},
  volume={350},
  number={6261},
  pages={659--662},
  year={2015},
  publisher={American Association for the Advancement of Science}
}

@article{Yan-2013,
  title={Observation of dipolar spin-exchange interactions with lattice-confined polar molecules},
  author={Yan, Bo and Moses, Steven A and Gadway, Bryce and Covey, Jacob P and Hazzard, Kaden RA and Rey, Ana Maria and Jin, Deborah S and Ye, Jun},
  journal={Nature},
  volume={501},
  number={7468},
  pages={521--525},
  year={2013},
  publisher={Nature Publishing Group}
}

@article{Hemmerich-1995,
  title={Trapping atoms in a dark optical lattice},
  author={Hemmerich, A and Weidem{\"u}ller, M and Esslinger, T and Zimmermann, C and H{\"a}nsch, T},
  journal={Physical review letters},
  volume={75},
  number={1},
  pages={37},
  year={1995},
  publisher={APS}
}

@article{Phillips-1985,
  title={Laser cooling and electromagnetic trapping of neutral atoms},
  author={Phillips, William D and Prodan, John V and Metcalf, Harold J},
  journal={JOSA B},
  volume={2},
  number={11},
  pages={1751--1767},
  year={1985},
  publisher={Optical Society of America}
}

@article{Balykin-1979,
  title={Observation of the cooling of free sodium atoms in a resonance laser field with a scanning frequency},
  author={Balykin, VI and Letokhov, VS and Mushin, VI},
  journal={JETP lett},
  volume={29},
  number={10},
  pages={560--564},
  year={1979}
}

@book{lucas-2013,
  title={Atomic and Molecular Beams: Production and Collimation},
  author={Lucas, Cyril Bernard},
  year={2013},
  publisher={CRC Press}
}

@article{Brune-2009,
  title={Thermal dynamics at surfaces},
  author={Brune, H},
  journal={Annalen der Physik},
  volume={18},
  number={10-11},
  pages={675--698},
  year={2009},
  publisher={Wiley Online Library}
}

@article{Bryden-1923,
  title={A Textbook of Filtration},
  author={Bryden, CL and Dickey, GD},
  journal={Easton, Pennsylvania},
  year={1923}
}

@book{Vickerman-2009,
  title={Surface analysis: the principal techniques},
  author={Vickerman, John C and Gilmore, Ian Stuart},
  volume={2},
  year={2009},
  publisher={Wiley Online Library}
}

@article{Moses-2010,
  title={Fabrication techniques and material properties of dielectric MgO thin films—a status review},
  author={Raj, A Moses Ezhil and Jayachandran, M and Sanjeeviraja, C},
  journal={CIRP Journal of Manufacturing Science and Technology},
  volume={2},
  number={2},
  pages={92--113},
  year={2010},
  publisher={Elsevier}
}

@article{Welton-1982,
  title={A LEED study of the MgO (100) surface: identification of a finite rumple},
  author={Welton-Cook, MR and Berndt, W},
  journal={Journal of Physics C: Solid State Physics},
  volume={15},
  number={27},
  pages={5691},
  year={1982},
  publisher={IOP Publishing}
}

@misc{Henrich-1994,
  title={The surface science of metal oxides, 1994},
  author={Henrich, VE and Cox, PA},
  publisher={Cambridge University Press, Cambridge}
}

@article{Gaddy-2014,
  title={Overcoming the polarization catastrophe in the rocksalt oxides MgO and CaO},
  author={Gaddy, Benjamin E and Paisley, Elizabeth A and Maria, Jon-Paul and Irving, Douglas L},
  journal={Physical Review B},
  volume={90},
  number={12},
  pages={125403},
  year={2014},
  publisher={APS}
}

@article{Coulomb-2013,
  title={Thermodynamic and structural properties of water adsorbed film on MgO (100) ionic surface},
  author={Coulomb, JP and Demirdjian, B and Ferry, D and Trabelsi, M},
  journal={Adsorption},
  volume={19},
  number={2-4},
  pages={861--867},
  year={2013},
  publisher={Springer}
}

@article{Freund-1996,
  title={Oxide surfaces},
  author={Freund, Hans-Joachim and Kuhlenbeck, Helmut and Staemmler, Volker},
  journal={Reports on Progress in Physics},
  volume={59},
  number={3},
  pages={283},
  year={1996},
  publisher={IOP Publishing}
}

@article{Debye-1912,
  title={Zur theorie der spezifischen w{\"a}rmen},
  author={Debye, Peter},
  journal={Annalen der Physik},
  volume={344},
  number={14},
  pages={789--839},
  year={1912},
  publisher={Wiley Online Library}
}
@article{Ashcroft-2010,
  title={Solid State Physics (Saunders College, Philadelphia, 1976)},
  author={Ashcroft, Neil W and Mermin, N David},
  journal={Appendix N},
  year={2010}
}

@article{Ferry-1998,
  title={Water monolayers on MgO (100): structural investigations by LEED experiments, tensor LEED dynamical analysis and potential calculations},
  author={Ferry, D and Picaud, S and Hoang, PNM and Girardet, C and Giordano, L and Demirdjian, B and Suzanne, J},
  journal={Surface science},
  volume={409},
  number={1},
  pages={101--116},
  year={1998},
  publisher={Elsevier}
}

@article{Blanchard-1991,
  title={A low-energy electron diffraction study of the MgO (001) surface structure},
  author={Blanchard, DL and Lessor, DL and LaFemina, JP and Baer, DR and Ford, WK and Guo, T},
  journal={Journal of Vacuum Science \& Technology A},
  volume={9},
  number={3},
  pages={1814--1819},
  year={1991},
  publisher={AVS: Science \& Technology of Materials, Interfaces, and Processing}
}
@article{Alford-2001,
  title={Dielectric loss of oxide single crystals and polycrystalline analogues from 10 to 320 K},
  author={Alford, N McN and Breeze, J and Wang, X and Penn, SJ and Dalla, S and Webb, SJ and Ljepojevic, N and Aupi, X},
  journal={Journal of the European Ceramic Society},
  volume={21},
  number={15},
  pages={2605--2611},
  year={2001},
  publisher={Elsevier}
}

@article{Stampe-1998,
  title={X-ray characterization of MgO thin films grown by laser ablation on yttria-stabilized zirconia},
  author={Stampe, Patricia A and Kennedy, Robin J},
  journal={Journal of crystal growth},
  volume={191},
  number={3},
  pages={472--477},
  year={1998},
  publisher={Elsevier}
}

@article{Harris-2013,
  title={Properties of an Infrared-Transparent MgO: Y2O3 Nanocomposite},
  author={Harris, Daniel C and Cambrea, Lee R and Johnson, Linda F and Seaver, Robert T and Baronowski, Meghan and Gentilman, Richard and Scott Nordahl, C and Gattuso, Todd and Silberstein, Stephanie and Rogan, Patrick and others},
  journal={Journal of the American Ceramic Society},
  volume={96},
  number={12},
  pages={3828--3835},
  year={2013},
  publisher={Wiley Online Library}
}

@article{Aswal-2002,
  title={XPS and AFM investigations of annealing induced surface modifications of MgO single crystals},
  author={Aswal, DK and Muthe, KP and Tawde, Shilpa and Chodhury, Sipra and Bagkar, N and Singh, Ajay and Gupta, SK and Yakhmi, JV},
  journal={Journal of crystal growth},
  volume={236},
  number={4},
  pages={661--666},
  year={2002},
  publisher={Elsevier}
}

@article{Yu-2003,
  title={Partial dissociation of water on a MgO (100) film},
  author={Yu, Yinghui and Guo, Qinlin and Liu, Shuang and Wang, Enge and M{\o}ller, Preben J},
  journal={Physical Review B},
  volume={68},
  number={11},
  pages={115414},
  year={2003},
  publisher={APS}
}

@article{Wlodarczyk-2011,
  title={Structures of the ordered water monolayer on MgO (001)},
  author={W{\l}odarczyk, Rados{\l}aw and Sierka, Marek and Kwapien, Karolina and Sauer, Joachim and Carrasco, Esther and Aumer, Andreas and Gomes, Janaina F and Sterrer, Martin and Freund, Hans-Joachim},
  journal={The Journal of Physical Chemistry C},
  volume={115},
  number={14},
  pages={6764--6774},
  year={2011},
  publisher={ACS Publications}
}

@article{Shin-2010,
  title={State-selective dissociation of a single water molecule on an ultrathin MgO film},
  author={Shin, Hyung-Joon and Jung, Jaehoon and Motobayashi, Kenta and Yanagisawa, Susumu and Morikawa, Yoshitada and Kim, Yousoo and Kawai, Maki},
  journal={Nature materials},
  volume={9},
  number={5},
  pages={442--447},
  year={2010},
  publisher={Nature Publishing Group}
}

@article{Goniakowski-1995,
  title={Theoretical investigation of hydroxylated oxide surfaces},
  author={Goniakowski, Jacek and Noguera, Claudine},
  journal={Surface science},
  volume={330},
  number={3},
  pages={337--349},
  year={1995},
  publisher={Elsevier}
}

@article{Johnson-1999,
  title={Dissociation of water at the MgO (100)-water interface: Comparison of theory with experiment},
  author={Johnson, Michael A and Stefanovich, Eugene V and Truong, Thanh N and G{\"u}nster, Jens and Goodman, DW},
  journal={The Journal of Physical Chemistry B},
  volume={103},
  number={17},
  pages={3391--3398},
  year={1999},
  publisher={ACS Publications}
}

@article{Guevara-Bertsch-2016,
  title={To be publish},
  author={Guevara-Bertsche, Milena and et al},
  year={2016},

}

@article{Batalhao-2015,
  title={Irreversibility and the arrow of time in a quenched quantum system},
  author={Batalhao, TB and Souza, AM and Sarthour, RS and Oliveira, IS and Paternostro, M and Lutz, E and Serra, RM},
  journal={Phys. Rev. Lett.},
   volume = {115},
  issue = {19},
  pages = {190601},
  numpages = {5},
  year = {2015},
 publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.115.190601},
  url = {http://link.aps.org/doi/10.1103/PhysRevLett.115.190601},
}

@article{Thissen-2012,
  title={pH-dependent structure and energetics of H 2 O/MgO (100)},
  author={Thissen, Peter and Thissen, Vera and Wippermann, Stefan and Chabal, Yves J and Grundmeier, Guido and Schmidt, Wolf Gero},
  journal={Surface Science},
  volume={606},
  number={11},
  pages={902--907},
  year={2012},
  publisher={Elsevier}
}

@book{MgOref-1999,
year={1999},
isbn={978-3-540-64964-9},
booktitle={II-VI and I-VII Compounds; Semimagnetic Compounds},
volume={41B},
series={Landolt-Börnstein - Group III Condensed Matter},
editor={Madelung, O. and Rössler, U. and Schulz, M.},
doi={10.1007/10681719_210},
title={Magnesium oxide (MgO) Young’s, shear and bulk moduli, Poisson’s ratio},
url={http://dx.doi.org/10.1007/10681719_210},
publisher={Springer Berlin Heidelberg},
keywords={Semiconductors; II-VI and I-VII Compounds; Semimagnetic Compounds},
pages={1-3},
language={English}
}


@article{Heidberg-1995,
  title={Adsorption of water vapor on the MgO (100) single crystal surface},
  author={Heidberg, Joachim and Redlich, Britta and Wetter, Dirk},
  journal={Berichte der Bunsengesellschaft f{\"u}r physikalische Chemie},
  volume={99},
  number={11},
  pages={1333--1337},
  year={1995},
  publisher={Wiley Online Library}
}

@article{Giordano-1998,
  title={Partial dissociation of water molecules in the (3$\times$ 2) water monolayer deposited on the MgO (100) surface},
  author={Giordano, Livia and Goniakowski, Jacek and Suzanne, Jean},
  journal={Physical review letters},
  volume={81},
  number={6},
  pages={1271},
  year={1998},
  publisher={APS}
}

@article{Jug-2007,
  title={Cyclic cluster study of water adsorption structures on the MgO (100) surface},
  author={Jug, Karl and Heidberg, Bettina and Bredow, Thomas},
  journal={Surface science},
  volume={601},
  number={6},
  pages={1529--1535},
  year={2007},
  publisher={Elsevier}
}

@book{Lu-2012,
  title={Applications of piezoelectric quartz crystal microbalances},
  author={Lu, Chao and Czanderna, Alvin Warren},
  year={2012},
  publisher={Elsevier}
}

@article{Sauerbrey-1959,
  title={Verwendung von Schwingquarzen zur W{\"a}gung d{\"u}nner Schichten und zur Mikrow{\"a}gung},
  author={Sauerbrey, G{\"u}nter},
  journal={Zeitschrift f{\"u}r physik},
  volume={155},
  number={2},
  pages={206--222},
  year={1959},
  publisher={Springer}
}

@article{Asano-1992,
  title={Mean atomic velocities of uranium, titanium and copper during electron beam evaporation},
  author={Asano, Takashi and Uetake, Naohito and Suzuki, Kazumichi},
  journal={Journal of Nuclear Science and Technology},
  volume={29},
  number={12},
  pages={1194--1200},
  year={1992},
  publisher={Taylor \& Francis}
}

@book{Haynes-2014,
  title={CRC handbook of chemistry and physics},
  author={Haynes, William M},
  year={2014},
  publisher={CRC press}
}

@book{Roth-2012,
  title={Vacuum technology},
  author={Roth, Alexander},
  year={2012},
  publisher={Elsevier}
}

@book{Johannsmann-2014,
  title={The Quartz Crystal Microbalance in Soft Matter Research},
  author={Johannsmann, Diethelm},
  year={2014},
  publisher={Springer}
}

@article{Pettersson-1919,
  title={Experiments with a new micro-balance},
  author={Pettersson, Hans},
  journal={Proceedings of the Physical Society of London},
  volume={32},
  number={1},
  pages={209},
  year={1919},
  publisher={IOP Publishing}
}

@inproceedings{Landis-1997,
  title={Dust on Mars: Materials adherence experiment results from Mars Pathfinder},
  author={Landis, Geoffrey and Jenkins, Phillip P and others},
  booktitle={Photovoltaic Specialists Conference, 1997., Conference Record of the Twenty-Sixth IEEE},
  pages={865--869},
  year={1997},
  organization={IEEE}
}

@book{Clarke-1985,
  title={Surface crystallography: an introduction to low energy electron diffraction},
  author={Clarke, Lionel J},
  year={1985},
  publisher={Wiley New York}
}

@article{Watson-1992,
  title={Critical Compilation of Surface Structures Determined by Surface Extended X-Ray Absorption Fine Structure (SEXAFS) and Surface Extended Electron Energy Loss Spectroscopy (SEELFS)},
  author={Watson, Philip R},
  journal={Journal of physical and chemical reference data},
  volume={21},
  number={1},
  pages={123--156},
  year={1992},
  publisher={AIP Publishing}
}

@article{Landman-1976,
  title={Extended x-ray-absorption fine structure—Auger process for surface structure analysis: Theoretical considerations of a proposed experiment},
  author={Landman, Uzi and Adams, David L},
  journal={Proceedings of the National Academy of Sciences},
  volume={73},
  number={8},
  pages={2550--2553},
  year={1976},
  publisher={National Acad Sciences}
}

@article{Citrin-1986,
  title={An overview of SEXAFS during the past decade},
  author={Citrin, PH},
  journal={Le Journal de Physique Colloques},
  volume={47},
  number={C8},
  pages={C8--437},
  year={1986},
  publisher={EDP Sciences}
}

@article{Lee-1976,
  title={Possibility of adsorbate position determination using final-state interference effects},
  author={Lee, PA},
  journal={Physical Review B},
  volume={13},
  number={12},
  pages={5261},
  year={1976},
  publisher={APS}
}

@article{Stern-1975,
  title={Extended x-ray-absorption fine-structure technique. III. Determination of physical parameters},
  author={Stern, EA and Sayers, DE and Lytle, FW},
  journal={Physical Review B},
  volume={11},
  number={12},
  pages={4836},
  year={1975},
  publisher={APS}
}

@book{Ibach-2013,
  title={Electron energy loss spectroscopy and surface vibrations},
  author={Ibach, Harald and Mills, Douglas L},
  year={2013},
  publisher={Academic Press}
}

@article{Woodruff-1988,
  title={From SEXAFS to SEELFS},
  author={Woodruff, DP},
  journal={Surface and Interface Analysis},
  volume={11},
  number={1-2},
  pages={25--35},
  year={1988},
  publisher={Wiley Online Library}
}

@article{Ehrenberg-1934,
  title={LXXXIII. A new method of investigating the diffraction of slow electrons by crystals},
  author={Ehrenberg, W},
  journal={The London, Edinburgh, and Dublin Philosophical Magazine and Journal of Science},
  volume={18},
  number={122},
  pages={878--901},
  year={1934},
  publisher={Taylor \& Francis}
}

@article{Scheibner-1960,
  title={Apparatus for Direct Observation of Low-Energy Electron Diffraction Patterns},
  author={Scheibner, EJ and Germer, LH and Hartman, CD},
  journal={Review of Scientific Instruments},
  volume={31},
  number={2},
  pages={112--114},
  year={1960},
  publisher={AIP Publishing}
}

@article{Park-1964,
  title={Pulsed-Beam Low Energy Electron Diffraction System for Rapid Precision Measurements},
  author={Park, Robert L and Farnsworth, HE},
  journal={Review of Scientific Instruments},
  volume={35},
  number={11},
  pages={1592--1596},
  year={1964},
  publisher={AIP Publishing}
}


@article{Mcrae-1964,
  title={Low-energy electron diffraction study of lithium fluoride (100) surface},
  author={McRae, EG and Caldwell, CW},
  journal={Surface Science},
  volume={2},
  pages={509--515},
  year={1964},
  publisher={Elsevier}
}

@article{Mcrae-1966,
  title={Multiple-Scattering Treatment of Low-Energy Electron-Diffraction Intensities},
  author={McRae, EG},
  journal={The Journal of Chemical Physics},
  volume={45},
  number={9},
  pages={3258--3276},
  year={1966},
  publisher={AIP Publishing}
}

@article{Holland-1971,
  title={A simple model for temperature effects in leed},
  author={Holland, BW},
  journal={Surface Science},
  volume={28},
  number={1},
  pages={258--266},
  year={1971},
  publisher={Elsevier}
}

@article{Hirabayashi-1968,
  title={Pseudopotential Approach to Diffraction Intensity of Low-Energy Electrons by Crystals},
  author={Hirabayashi, Kanji},
  journal={Journal of the Physical Society of Japan},
  volume={24},
  number={4},
  pages={846--854},
  year={1968},
  publisher={The Physical Society of Japan}
}

@article{Tong-1975,
  title={Theory of low-energy electron diffraction},
  author={Tong, Shuk Y},
  journal={Progress in surface science},
  volume={7},
  number={1},
  pages={1--48},
  year={1975},
  publisher={Elsevier}
}

@article{Yang-2015,
  title={A high flux source of cold strontium atoms},
  author={Yang, T and Pandey, K and Pramod, MS and Leroux, F and Kwong, CC and Hajiyev, E and Chia, ZY and Fang, B and Wilkowski, D},
  journal={arXiv preprint arXiv:1505.04507},
  year={2015}
}

@article{kasemo1979kinetics,
  title={The kinetics of hydrogen interaction with TiHx films, 0≤ x≲ 2},
  author={Kasemo, B and T{\"o}rnqvist, E},
  journal={Applications of Surface Science},
  volume={3},
  number={3},
  pages={307--328},
  year={1979},
  publisher={Elsevier}
}

@article{huang1987statistical,
  title={Statistical Mechanics, 2nd},
  author={Huang, Kerson},
  journal={Edition (New York: John Wiley \& Sons)},
  year={1987}
}

@book{lu2012applications,
  title={Applications of piezoelectric quartz crystal microbalances},
  author={Lu, Chao and Czanderna, Alvin Warren},
  volume={7},
  year={2012},
  publisher={Elsevier}
}
@article{zinzi2011exploring,
  title={Exploring the feasibility of volatile desorption studies by means of a quartz crystal microbalance with an integrated micro-heater},
  author={Zinzi, Angelo and Palomba, Ernesto and Zampetti, Emiliano and Pantalei, Simone and Longobardo, Andrea and Macagnano, Antonella and Bearzotti, Andrea},
  journal={Sensors and Actuators A: Physical},
  volume={172},
  number={2},
  pages={504--510},
  year={2011},
  publisher={Elsevier}
}

@article{kurosawa2000detection,
  title={Detection of deposition rate of plasma-polymerized films by quartz crystal microbalance},
  author={Kurosawa, Shigeru and Hirokawa, Tomoya and Kashima, Kazuya and Aizawa, Hidenobu and Han, Dae-Sang and Yoshimi, Yasuo and Okada, Yuji and Yase, Kiyoshi and Miyake, Jun and Yoshimoto, Minoru and others},
  journal={Thin Solid Films},
  volume={374},
  number={2},
  pages={262--267},
  year={2000},
  publisher={Elsevier}
}

@article{leskela2002atomic,
  title={Atomic layer deposition (ALD): from precursors to thin film structures},
  author={Leskel{\"a}, Markku and Ritala, Mikko},
  journal={Thin solid films},
  volume={409},
  number={1},
  pages={138--146},
  year={2002},
  publisher={Elsevier}
}

@article{yousfi2001atomic,
  title={Atomic layer deposition of zinc oxide and indium sulfide layers for Cu (In, Ga) Se 2 thin-film solar cells},
  author={Yousfi, EB and Weinberger, B and Donsanti, F and Cowache, P and Lincot, D},
  journal={Thin Solid Films},
  volume={387},
  number={1},
  pages={29--32},
  year={2001},
  publisher={Elsevier}
}

@article{kasemo1978quartz,
  title={Quartz crystal microbalance measurements of O/Ti and CO/Ti atom ratios on very thin Ti films},
  author={Kasemo, B and T{\"o}rnqvist, E},
  journal={Surface science},
  volume={77},
  number={2},
  pages={209--218},
  year={1978},
  publisher={Elsevier}
}

@article{mecea2006fundamentals,
  title={Fundamentals of mass measurements},
  author={Mecea, V},
  journal={Journal of thermal analysis and calorimetry},
  volume={86},
  number={1},
  pages={9--16},
  year={2006},
  publisher={Akad{\'e}miai Kiad{\'o}, co-published with Springer Science+ Business Media BV, Formerly Kluwer Academic Publishers BV}
}

@article{meyer1981thermalization,
  title={Thermalization of sputtered atoms},
  author={Meyer, Kevin and Schuller, Ivan K and Falco, Charles M},
  journal={Journal of Applied Physics},
  volume={52},
  number={9},
  pages={5803--5805},
  year={1981},
  publisher={AIP}
}

@article{rendulic1994adsorption,
  title={Adsorption and desorption dynamics as seen through molecular beam techniques},
  author={Rendulic, KD and Winkler, A},
  journal={Surface science},
  volume={299},
  pages={261--276},
  year={1994},
  publisher={Elsevier}
}

@article{yang2014atomic,
  title={Atomic scale calculations of tungsten surface binding energy and beryllium-induced tungsten sputtering},
  author={Yang, Xue and Hassanein, Ahmed},
  journal={Applied Surface Science},
  volume={293},
  pages={187--190},
  year={2014},
  publisher={Elsevier}
}

@article{kudriavtsev2005calculation,
  title={Calculation of the surface binding energy for ion sputtered particles},
  author={Kudriavtsev, Yu and Villegas, A and Godines, A and Asomoza, R},
  journal={Applied surface science},
  volume={239},
  number={3-4},
  pages={273--278},
  year={2005},
  publisher={Elsevier}
}

@article{redhead1962thermal,
  title={Thermal desorption of gases},
  author={Redhead, PA},
  journal={Vacuum},
  volume={12},
  number={4},
  pages={203--211},
  year={1962},
  publisher={Elsevier}
}

@article{king1975thermal,
  title={Thermal desorption from metal surfaces: A review},
  author={King, David A},
  journal={Surface Science},
  volume={47},
  number={1},
  pages={384--402},
  year={1975},
  publisher={Elsevier}
}

@article{bourgoin2010thermal,
  title={Thermal conduction in thin films measured by optical surface thermal lensing},
  author={Bourgoin, Jean-Philippe and Allogho, Guy-Germain and Hach{\'e}, Alain},
  journal={Journal of Applied Physics},
  volume={108},
  number={7},
  pages={073520},
  year={2010},
  publisher={AIP}
}

@article{martan2006thermal,
  title={Thermal characterization of tungsten thin films by pulsed photothermal radiometry},
  author={Martan, Jiri and Semmar, Nadjib and Boulmer-Leborgne, Chantal and Plantin, Pascale and Le Menn, Erwan},
  journal={Nanoscale and Microscale Thermophysical Engineering},
  volume={10},
  number={4},
  pages={333--344},
  year={2006},
  publisher={Taylor \& Francis}
}

@article{kim2007spray,
  title={Spray cooling heat transfer: the state of the art},
  author={Kim, Jungho},
  journal={International Journal of Heat and Fluid Flow},
  volume={28},
  number={4},
  pages={753--767},
  year={2007},
  publisher={Elsevier}
}

@article{hansch2006einstein,
  title={Einstein Lecture--Passion for precision},
  author={H{\"a}nsch, Theodor W},
  journal={Annalen der Physik},
  volume={15},
  number={9},
  pages={627--652},
  year={2006},
  publisher={Wiley Online Library}
}

@article{hagena1968time,
  title={Time-of-Flight Velocity Analysis of Atomic and Molecular Beams},
  author={Hagena, Otto F and Varma, Ashok K},
  journal={Review of Scientific Instruments},
  volume={39},
  number={1},
  pages={47--52},
  year={1968},
  publisher={AIP}
}

@article{phillips1998nobel,
  title={Nobel Lecture: Laser cooling and trapping of neutral atoms},
  author={Phillips, William D},
  journal={Reviews of Modern Physics},
  volume={70},
  number={3},
  pages={721},
  year={1998},
  publisher={APS}
}

@article{guggemos2015sympathetic,
  title={Sympathetic cooling and detection of a hot trapped ion by a cold one},
  author={Guggemos, Michael and Heinrich, Daniel and Herrera-Sancho, Oscar A and Blatt, Rainer and Roos, Christian Felix},
  journal={New Journal of Physics},
  volume={17},
  number={10},
  pages={103001},
  year={2015},
  publisher={IOP Publishing}
}

@article{nicholson2015systematic,
  title={Systematic evaluation of an atomic clock at 2$\times$ 10- 18 total uncertainty},
  author={Nicholson, TL and Campbell, SL and Hutson, RB and Marti, GE and Bloom, BJ and McNally, RL and Zhang, Wei and Barrett, MD and Safronova, MS and Strouse, GF and others},
  journal={Nature communications},
  volume={6},
  pages={6896},
  year={2015},
  publisher={Nature Publishing Group}
}

@article{ludlow2015optical,
  title={Optical atomic clocks},
  author={Ludlow, Andrew D and Boyd, Martin M and Ye, Jun and Peik, Ekkehard and Schmidt, Piet O},
  journal={Reviews of Modern Physics},
  volume={87},
  number={2},
  pages={637},
  year={2015},
  publisher={APS}
}

@article{safronova2018two,
  title={Two clock transitions in neutral Yb for the highest sensitivity to variations of fundamental constants},
  author={Safronova, MS and Porsev, SG and Sanner, Christian and Ye, Jun},
  journal={arXiv preprint arXiv:1801.06239},
  year={2018}
}

@article{kolkowitz2016gravitational,
  title={Gravitational wave detection with optical lattice atomic clocks},
  author={Kolkowitz, Shimon and Pikovski, Igor and Langellier, Nicholas and Lukin, Mikhail D and Walsworth, Ronald L and Ye, Jun},
  journal={Physical Review D},
  volume={94},
  number={12},
  pages={124043},
  year={2016},
  publisher={APS}
}

@article{reichelt1990preparation,
  title={The preparation of thin films by physical vapour deposition methods},
  author={Reichelt, K and Jiang, X},
  journal={Thin Solid Films},
  volume={191},
  number={1},
  pages={91--126},
  year={1990},
  publisher={Elsevier}
}

@article{rosenband2007observation,
  title={Observation of the S 0 1→ P 0 3 Clock Transition in Al+ 27},
  author={Rosenband, Till and Schmidt, Piet O and Hume, David B and Itano, Wayne M and Fortier, Tara M and Stalnaker, Jason E and Kim, K and Diddams, Scott A and Koelemeij, JCJ and Bergquist, JC and others},
  journal={Physical review letters},
  volume={98},
  number={22},
  pages={220801},
  year={2007},
  publisher={APS}
}

@article{nicholson2012comparison,
  title={Comparison of two independent Sr optical clocks with 1$\times$ 10- 17 stability at 10 3 s},
  author={Nicholson, TL and Martin, MJ and Williams, JR and Bloom, BJ and Bishof, M and Swallows, MD and Campbell, SL and Ye, J},
  journal={Physical review letters},
  volume={109},
  number={23},
  pages={230801},
  year={2012},
  publisher={APS}
}

@article{itano2000external,
  title={External-field shifts of the 199Hg+ optical frequency standard},
  author={Itano, Wayne M},
  journal={Journal of research of the National Institute of Standards and Technology},
  volume={105},
  number={6},
  pages={829},
  year={2000},
  publisher={National Institute of Standards and Technology}
}

@article{chou2010optical,
  title={Optical clocks and relativity},
  author={Chou, Chin-Wen and Hume, DB and Rosenband, Till and Wineland, DJ},
  journal={Science},
  volume={329},
  number={5999},
  pages={1630--1633},
  year={2010},
  publisher={American Association for the Advancement of Science}
}

@article{schmidt2001nanotechnology,
  title={Nanotechnology: Thin solid films roll up into nanotubes},
  author={Schmidt, Oliver G and Eberl, Karl},
  journal={Nature},
  volume={410},
  number={6825},
  pages={168},
  year={2001},
  publisher={Nature Publishing Group}
}

@article{beyertt2005optical,
  title={Optical in-well pumping of a semiconductor disk laser with high optical efficiency},
  author={Beyertt, S-S and Zorn, Martin and Kubler, T and Wenzel, Hans and Weyers, Markus and Giesen, Adolf and Trankle, GATG and Brauch, Uwe},
  journal={IEEE journal of quantum electronics},
  volume={41},
  number={12},
  pages={1439--1449},
  year={2005},
  publisher={IEEE}
}

@article{saas2006exciton,
  title={Exciton resonance tuning for the generation of subpicosecond pulses from a mode-locked semiconductor disk laser},
  author={Saas, Florian and Steinmeyer, G{\"u}nter and Griebner, Uwe and Zorn, Martin and Weyers, Markus},
  journal={Applied physics letters},
  volume={89},
  number={14},
  pages={141107},
  year={2006},
  publisher={AIP}
}

@article{guevara2016detection,
  title={Detection of the adsorption of water monolayers through the ion oscillation frequency in the magnesium oxide lattice by means of low energy electron diffraction},
  author={Guevara-Bertsch, Milena and Ram{\'\i}rez-Hidalgo, Gustavo and Chavarr{\'\i}a-Sibaja, Andr{\'e}s and Avenda{\~n}o, E and Araya-Pochet, Jose A and Herrera-Sancho, Oscar A },
  journal={AIP Advances},
  volume={6},
  number={3},
  pages={035317},
  year={2016},
  publisher={AIP Publishing}
}

@article{kasemo2002biological,
  title={Biological surface science},
  author={Kasemo, Bengt},
  journal={Surface science},
  volume={500},
  number={1-3},
  pages={656--677},
  year={2002},
  publisher={Elsevier}
}

@book{freund2004thin,
  title={Thin film materials: stress, defect formation and surface evolution},
  author={Freund, Lambert Ben and Suresh, Subra},
  year={2004},
  publisher={Cambridge University Press}
}

@book{pamplin2017molecular,
  title={Molecular beam epitaxy},
  author={Pamplin, Brian R},
  year={2017},
  publisher={Elsevier}
}


@article{moylan2003new,
  title={A new approach for studying mechanical properties of thin surface layers affected by manufacturing processes},
  author={Moylan, SP and Kompella, S and Chandrasekar, S and Farris, TN},
  journal={Journal of manufacturing science and engineering},
  volume={125},
  number={2},
  pages={310--315},
  year={2003},
  publisher={American Society of Mechanical Engineers}
}

@book{mattox2010handbook,
  title={Handbook of physical vapor deposition (PVD) processing},
  author={Mattox, Donald M},
  year={2010},
  publisher={William Andrew}
}


@article{wadley2001mechanisms,
  title={Mechanisms, models and methods of vapor deposition},
  author={Wadley, HNG and Zhou, X and Johnson, RA and Neurock, M},
  journal={Progress in Materials Science},
  volume={46},
  number={3-4},
  pages={329--377},
  year={2001},
  publisher={Elsevier}
}

@article{aspnes1982optical,
  title={Optical properties of thin films},
  author={Aspnes, David E},
  journal={Thin solid films},
  volume={89},
  number={3},
  pages={249--262},
  year={1982},
  publisher={Elsevier}
}

@article{gravitationalwaves,
  title = {GW170817: Observation of Gravitational Waves from a Binary Neutron Star Inspiral},
  author = { Abbott,Bart P and  al},
  collaboration = {LIGO Scientific Collaboration and Virgo Collaboration},
  journal = {Phys. Rev. Lett.},
  volume = {119},
  issue = {16},
  pages = {161101},
  numpages = {18},
  year = {2017},
  month = {Oct},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.119.161101},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.119.161101}
}

@article{herrera2011ultra,
  title={Ultra thin films of gadolinium deposited by evaporation in ultra high vacuum conditions: Composition, growth and morphology},
  author={Herrera-Sancho, Oscar A and Castro-Gonz{\'a}lez, Diego and Araya-Pochet, Jose A and Vargas-Castro, WE},
  journal={Applied Surface Science},
  volume={257},
  number={8},
  pages={3510--3518},
  year={2011},
  publisher={Elsevier}
}
